Spatial Reasoning via Deep Vision Models for Robotic Sequential Manipulation

In this paper, we propose using deep neural architectures (i.e., vision transformers and ResNet) as heuristics for sequential decision-making in robotic manipulation problems. This formulation enables predicting the subset of objects that are relevant for completing a task. Such problems are often addressed by task and motion planning (TAMP) formulations combining symbolic reasoning and continuous motion planning. In essence, the action-object relationships are resolved for discrete, symbolic decisions that are used to solve manipulation motions (e.g., via nonlinear trajectory optimization). However, solving long-horizon tasks requires consideration of all possible action-object combinations which limits the scalability of TAMP approaches. To overcome this combinatorial complexity, we introduce a visual perception module integrated with a TAMP-solver. Given a task and an initial image of the scene, the learned model outputs the relevancy of objects to accomplish the task. By incorporating the predictions of the model into a TAMP formulation as a heuristic, the size of the search space is significantly reduced. Results show that our framework finds feasible solutions more efficiently when compared to a state-of-the-art TAMP solver.

==> 9_Todo_list.tex <==
\newpage
\section{Check list}

\begin{CheckList}{Goal}
\Goal{open}{Reviews from 11495}
  \begin{CheckList}{Task}
     \Task{done}{The specific difficulty of the task goal was not explained clearly. I don't know how many steps it takes to complete a task in the experiments.}
     - Usually there are 4 steps for achieving the goal. Namly, 1. pickup the object which occupied the target localtion. 2. place the object on any other position other than the target location. 3. pick up the target object. 4. place the target object on target location.
     \Task{done}{Are there any failure cases? In the experimental results, the authors show the computational speed of LGP. And how to measure the quality of the computed action sequences.}
     - There are failure cases due to the time limitation, which means the LGP is not efficient enough to solve the problem within the time limitation. The quality of the action sequences is optimized by LGP under pre-defined constraints. This means, as long as the constraints didn't change, we will get the results with the same quality.
     \Task{done}{Can this method handle situations where objects are completely occluded? If there are task-related objects that cannot be observed at the beginning, during task execution, the occluded objects can be included in the TAMP solver based on new observations?}
     - Sadly, no, since the framework is offline, I'm not able to update/modify the optimization strategy on the fly.
     \Task{done}{How to solve the problem of the same color of blocks? If there are multiple identical blocks, how will the model behave?}
     - In this case, the model will not be able to recognize the objects specified by the query. Due to the Attention-based nature of the Transformer, it is reasonable to assume that the Transformer will give similar results for the same objects. 
     
     - The model will output positive if one of the object which shared same outlook is relevant (verified with experiment).
     \Task{done}{Experiments show that the classification results of different classifier structures are not significantly different. No further in-depth analysis. The current results do not reflect the value of multiple network structures for classification. There is a lack of ablation experiments to demonstrate which parts are critical to classification results. In other words, is a generic classification structure sufficient for such a simple classification task. Therefore, I think it is necessary to increase the difficulty of tasks such as the diversity of the background and the difference in lighting, which will challenge the generalization of visual models, and in turn reflect the value of different network structures.}
     - Limited by the framework. :(
  \end{CheckList}

\Goal{open}{Reviews from 24203}
    \begin{CheckList}{Task}
         \Task{done}{1. The “spatial relationship” between two objects is not defined in the paper. Is it the same as the relevance of an object given a goal predicate?}
         - Yes, the spatial relationship is a state between two objects which can be described by one or multiple predicate.
         \Task{done}{2. Does the goal state only contain one predicate? E.g., object A is on-the-left of B. In a TAMP problem, there can usually be more than one predicate in the goals states. For example, object A is on-the-left of B \& object C is on-top of B.}
         - Yes, the goal state only contain one predicate. 
         \Task{open}{3. In contribution 2, the authors mention a “scalable predicate extractor.” While this probably refers to the multi-head model in Sec. VI. The authors do not clearly define scalability in the paper. If multiple predicates exist in the goal state, will the framework still be scalable?}
         - Theoretically, the model should be scalable, if multiple predicates exist.
         \Task{done}{4. Some of the equations $(1b)-(1i)$ are not referenced in the text. The equations should be explained one by one for clarity. As an example, the function $A(s_{k-1}, S)$ in $(1e)$ is not defined.}
         \Task{done}{5. “The $\theta(a)$ takes an action as parameter and retrieves the object involved in the action.” Is it correct that the function $\theta(a)$ only returns one object involved in the action? Seems there is an assumption that all actions are single objective actions and should be made explicit.}
         \Task{done}{6. It is unclear how the ground truth labels are obtained for training and testing.}
         - The calculation is done by LGP, but with a significantly higher upper time limit to ensure that a result will be found.
         \Task{done}{7. How long does it take to train the networks?}
         - Each Predicate Extractor was trained by using two RTX 3090 graphics card for 48 hours and 20 epochs.
         \Task{open}{8. In Sec. VI Experiments, it would be great to know the number of objects in the cases in the dataset. In addition, the framework is useful when there are many objects in the case. Is the learning model able to predict relevance when there is a large number of objects? Will the speed-up percentage be larger when there are more objects in the cases?}
         - The datasets are created with 10 different object in terms of the shape and color. (I didn't test this part. Since I'm not sure with the generalizability of the model. But I did trained a model for 6 objects. Maybe I should compare between these two models?)
         \Task{done}{9. “If the prediction $t(I,p0,...L,qi)$ for object i is higher than the threshold $\beta \in \mathcal{R}$, then we decide that $ZS(i) = 1$, i.e., the object is relevant to the action sequence.” “As $\beta$ increases, the model will adopt a more conservative strategy so that more data will be marked as relevant.” I feel these two sentences are inconsistent with each other. I.e., according to the former sentence, the model should mark fewer objects as relevant if $\beta$ increases.}
         \Task{open}{10. In Fig. 8, why is the range of $\beta$ only 0-0.1 while the probability of the relevance can range from 0-1? Why is there still speed up when $\beta = 0$ (as all objects will be considered relevant)? Also, according to Fig. 8, the speed-up does not change much when the $\beta$ changes. I.e., we don’t see a clear trend of larger speed-up when changing $\beta$. Is there any explanation?}
         - Because collecting these data needs to run LGP one by one. And the LGP consumes a lot of time. We didn't see a clear trend of speed-up, because the $\Delta\beta$ is still too low to see the change. Also the results came from the model for on-top predicate which is already very hard task for the model, our experiment by changing the $\beta$ maybe still not reaching the point where the model consider whether an object is relevant or not.
         \Task{done}{11. What will happen if the canonical view is much different from the view in the scene? I.e., is the predicted relevance going to change much when the objects in the scene are viewed from a different angle? A robustness analysis could strengthen the paper.}
         - We sample the canonical views from randomized angles, these canonical views are randomly picked during the training. Therefore, even the canonical views in the query are much different from the object in the scene, the model will still be able to recognize the object.
         \Task{done}{Please add a bracket around the equations. Sometimes it is quite confusing without the bracket. For example, “mixed-integer program 1” and “learned classifier 4”.}
    \end{CheckList}

\Goal{open}{Rephrase}
    \begin{CheckList}{Task}
        \Task{done}{Section III}
    \end{CheckList}

\end{CheckList}
